A Reliability-aware Multi-armed Bandit Approach to Learn and Select Users in Demand Response

One challenge in the optimization and control of societal systems is to handle the unknown and uncertain user behavior. This paper focuses on residential demand response (DR) and proposes a closed-loop learning scheme to address these issues. In particular, we consider DR programs where an aggregator calls upon residential users to change their demand so that the total load adjustment is close to a target value. To learn and select the right users, we formulate the DR problem as a combinatorial multi-armed bandit (CMAB) problem with a reliability objective. We propose a learning algorithm: CUCB-Avg (Combinatorial Upper Confidence Bound-Average), which utilizes both upper confidence bounds and sample averages to balance the tradeoff between exploration (learning) and exploitation (selecting). We consider both a fixed time-invariant target and time-varying targets, and show that CUCB-Avg achieves $O(\log T)$ and $O(\sqrt{T \log(T)})$ regrets respectively. Finally, we numerically test our algorithms using synthetic and real data, and demonstrate that our CUCB-Avg performs significantly better than the classic CUCB and also better than Thompson Sampling.

==> arxiv submit/sec1_introduction.tex <==
\section{Introduction}

%\paragraph{Draft.}
Unknown and uncertain user behavior is common in many sequential decision-making problems of societal systems, such as transportation, electricity grids, communication, crowd-sourcing, and resource allocation problems in general \citep{o2010residential,belleflamme2014crowdfunding,kuderer2015learning,li2017mechanism}. One key challenge caused by the unknown and uncertain user behavior is how to ensure reliability or reduce risks for the system.  This paper focuses on addressing this challenge for residential demand response (DR) in power systems.
 
 
 Residential DR refers to adjusting  power consumption of residential users, e.g. by changing the temperature setpoints of air conditioners,  to relieve  the supply-demand imbalances of the power system \citep{DRreportFERC2017,conEdison,o2010residential,thinkeco,psegcoolcustomer}. In most residential DR programs, customers can decide to respond to a DR signal or not, and the decisions are usually highly uncertain. Moreover, the pattern of the user behavior is not well understood by the DR aggregator. Such unknown and uncertain behavior may cause severe troubles for the system reliability: without enough knowledge of the user behavior,  the DR load adjustment  is likely to be very different from a target level, resulting in extra power imbalances and fluctuations. Therefore, it is critical for residential DR programs to learn the user behavior and ensure reliability  during the learning. 
 
 
 %are very different from the desirable load adjustment that is needed by the power system, which will cause extra supply-demand imbalance and extra variation and fluctuations. Now, to effectively apply residential DR, a critical question is how to learn the customers and how to ensure reliability of the program during the learning. 
 
 
 Multi-armed bandit (MAB) emerges as a natural framework to learn the user  behavior \citep{auer2002finite,bubeck2012regret}.  In a simple setting, MAB considers $n$ independent arms, each providing a random contribution according to its own distribution at time step $1\leq t \leq T$. 
 Without knowing these distributions, a decision maker picks one arm at each time step and tries to maximize the total expected contribution in $T$ time steps. %The decision maker  decides whether to \textit{explore} arms to learn the unknown distributions, or to \textit{exploit} the current knowledge by selecting the arm with highest mean contribution so far.
  When the decision maker can select multiple arms at each time, the problem is often referred to as  combinatorial multi-armed bandit (CMAB) in literature \citep{chen2016combinatorial,kveton2015tight}.  (C)MAB captures a fundamental tradeoff in most learning problems: \textit{exploration} vs. \textit{exploitation}. A common metric to evaluate the performance of (C)MAB learning algorithms is regret, which captures the difference between  the optimal expected value assuming the distributions are known and the  expected value achieved by the online learning algorithm. It is desirable to design online algorithms with sublinear $o(T)$ regrets, which roughly indicates that  the learning algorithm eventually learns the optimal solution.
  %The goal is to design online algorithms with sublinear $o(T)$ regrets, 
  
  %In literature, 
% a sublinear $o(T)$ regret is usually desirable implies good performance since it indicates that the learning algorithm eventually learns the optimal solution.
 
 
% When applying CMAB framework to residential demand response, we can treat each customer as one arm. Then the aggregator follows CMAB methods to explore (learn) and exploit (select) the customers to achieve the goal of its DR program. 
 
  Though there have been studies on DR via  (C)MAB, most literature aims at maximizing the load reduction \citep{wang2014adaptive,lesage2017multi,jain2014multiarmed}. There is a lack of efforts on improving the reliability of CMAB algorithms for DR as well as the theoretical reliability guarantees. 
  
%  sets the goal as maximizing the load reduction for peak hours rather than following a load reduction target for reliability concerns. There is also a lack of theoretical guarantee for the reliability of CMAB algorithms in DR.} %Besides, conducting rigorous regret analysis for achieving sub-linear regret is always challenging. 
  
  

\subsection{Our Contributions} 
In this paper, we formulate the DR as a CMAB problem with a reliability objective, i.e. we aim to minimize the deviation between the actual total load adjustment and a target signal. The target might be caused by a sudden change of renewable energy or a peak load reduction event.   We consider a large number of residential users, and each user can commit one unit of load change (either reduction or increase) with an unknown probability. The task of the DR aggregator is to select a subset of the users to guarantee the actual load adjustment to be as close to the target as possible. The number of  users to select is not fixed, giving flexibility to the aggregator for achieving different target levels.  %Compared with the classic CMAB literature \citep{chen2016combinatorial,combes2015combinatorial,gai2012combinatorial,kveton2014matroid,kveton2015tight}, a major difference of our formulation is that the reliability objective leads to a non-monotonic objective, rendering the existing CMAB approaches and regret analysis inapplicable here \citep{chen2016combinatorial}. 


In order to design our  online learning algorithm, we first develop an offline combinatorial optimization algorithm that selects the optimal subset of the users when the user behavior models are known. Based 
on the structure of the offline algorithm, we propose an online algorithm CUCB-Avg (Combinatorial Upper Confidence Bound-Average) and provide a rigorous regret analysis.  We show that, over $T$ time steps,  CUCB-Avg achieves $O(\log T)$ regret given a static target and $O(\sqrt{T\log(T)}$ regret given a time-varying target. The regrets in both cases depend polynomially on the number of users $n$. We also conduct numerical studies using synthetic DR data, showing that the performance of CUCB-Avg is much better than the classic algorithm CUCB \citep{kveton2015tight,chen2016combinatorial}, and also better than  Thompson sampling. % another popular CMAB method which uses a Bayesian learning approach and has good empirical performance \citep{russo2017tutorial,agrawal2012analysis,chapelle2011empirical}. 
In addition, we numerically show that, with minor modifications,  CUCB-Avg can cope with more realistic  behavior models with user fatigue. 



Lastly, we would like to mention that though the DR model considered in this paper is very simple, the model is motivated by real pilot studies of residential DR programs, and the results have served as a guideline for designing the learning protocols \citep{thinkeco}. Besides, since real-world DR programs vary a lot among each other (depending on the DR company, local policies, reward schemes, data infrastructure, etc.), abstracting the DR model can be useful for a variety of DR programs by providing some common insights and general guidelines. When designing algorithms for real DR programs, we could modify the vanilla method to suit different specific requirements. 
 Furthermore, our algorithm design and  theoretical analysis based on the simple model may also provide insights for  other societal system applications.
 
 % the DR model in this paper appears simplified compared to real-world DR programs, 
% the model was motivated by real-world field studies of residential DR and the results in this paper have served as a guideline to design learning protocols for these studies \citep{conEdison}. Moreover, through modifying the detailed algorithms for other applications, the overall closed-loop learning scheme  and the technical tools for analyzing its theoretical performance are useful for other societal systems especially with human-in-the-loop.
 %, though the algorithms would require modifications for different applications. 
 % via modifying the detailed algorithm for different applications. 
 %, though the algorithm might require modifications for different applications.

\subsection{Related Work}
\textit{Combinatorial multi-armed bandits.}
 Most literature in CMAB studies a classic formulation which aims to maximize the total (weighted) contribution of $K$ arms with a \textit{fixed} integer $K$ (and known weights) \citep{bubeck2012regret,kveton2015tight}. 
There are also papers considering more general reward functions, for example, \citep{chen2016combinatorial} considers   objective functions that are \textit{monotonically nondecreasing}  with the parameters of the selected arms and designs Combinatorial Upper Confidence Bound (CUCB) using the principle of \textit{optimism in the face of uncertainty}.
%settings where the goal is to select a subset of arms to maximize some reward functions, for example, \citep{chen2016combinatorial} designs Combinatorial Upper Confidence Bound (CUCB) using the principle of \textit{optimism in the face of uncertainty} when the objective function is \textit{monotonically nondecreasing} with the parameters of arms given a fixed selected subset. 
However, the reliability objective of our CMAB problem does not satisfy the monotonicity assumption, thus the study of CUCB  cannot be directly applied here. %\lina{I am some confused by the flow/meaning for the former two sentences. ``As for more general settings, ...'', which is the more general? Does that paper studies super arm, base arms etc? Or do you want to say for general objective function but the objective function is nondecreasing? }
Another line of work follows the \textit{Bayesian} approach and studies Thompson sampling \citep{gopalan2014thompson,wang2018thompson}. \red{However, the regret bound of Thompson sampling consists of a term that is independent of $T$ but depends  exponentially on the number of   arms $K$ in the optimal subset \citep{wang2018thompson}. Further,  \citep{wang2018thompson} shows that the exponential dependence is unavoidable. In  the residential DR problems, $K$ is usually large, so Thompson sampling may generate poor performance especially when $T$ is not very large, which is consistent with our numerical results in Figure \ref{fig: compare TS with diff. n} in Section \ref{sec: simulation}.} Finally, there is a lack of analysis on time-varying objective functions, but in many real-world applications the objectives change with time, e.g., the DR target would depend on the time-varying renewable generation. Therefore, either the learning algorithms or the theoretical analysis in literature do not directly apply to our CMAB problem, motivating the work of this paper.


\textit{Risk-aversion MAB.} There is a related line of  research on reducing risks in MAB by  selecting the \textit{single} arm with the best \textit{return-risk tradeoff} \citep{sani2012risk,vakili2016risk}.  However, there is a  lack of studies on selecting \textit{a subset of} arms so that the total contribution of the selected arms is \textit{close to a certain target.\footnote{\red{In Appendix \ref{append: risk averse}, we provide an algorithm based on the risk-aversion MAB ideas and provide numerical results.}}}
	
	%Risk-aversion or risk-aware MAB is a related line of research on reducing risks in MAB \citep{sani2012risk,vakili2016risk}. Most  papers on risk-aversion MAB focus on selecting the  \textit{single} arm with the best \textit{return-risk tradeoff}, where the return is measured by the expectation of the reward and the risk is measured by the variance. However, there is a lack of studies on selecting \textit{a subset of} arms so that the total contribution is \textit{close to a certain target}, which is the focus of this paper.}


\textit{Learning-based demand response.} In addition to the demand response program considered in this paper and \citep{wang2014adaptive,lesage2017multi,thinkeco,psegcoolcustomer,conEdison}, where customers are directly selected by the aggregator to  perform demand response, there is a different type of DR programs based on dynamic pricing,  where the goal is to design time-varying electricity prices to automatically incentivize  desirable load reduction behaviors from the consumers  \citep{dynamicpricing}. Learning-based algorithms are also proposed for this type of DR programs to deal with, for example, the unknown utility functions of the consumers \citep{khezeli2017risk,li2017distributed,moradipari2018learning}.  



%iii) other DR and learning, incentive design. Including mechanism design, and pricing sheme design.

%%\blue{rewrite it, I deleted the incentive part, so I may need to include it here.}
%\textcolor{blue}{Another related line of work on learning-based demand response is based on dynamic pricing demand response programs, where the goal is to design time-varying electricity prices as incentives for desirable load reduction behaviors by learning  consumers' utility functions \citep{khezeli2017risk,li2017distributed,moradipari2018learning}. This is different from the DR schemes considered in this paper and \citep{wang2014adaptive,lesage2017multi} whose task is to  select the right group of consumers by learning the behavior patterns of consumers under a potentially fixed payment rule. Both DR schemes enjoy many real-world programs and pilot studies, e.g.  some dynamic pricing pilots are summarized in \citep{dynamicpricing} and customer-selection-type DR usually finds its applications in smart air conditioner programs \citep{thinkeco,psegcoolcustomer,dukeenergywisehome}.}

%to be close to a certain target, which is the focus on this paper.

%There are papers on risk control in MAB, which is usually called as risk-aversion MAB (cite??). They usually measure risks by variance and aim to select the single arm with the best return-risk tradeoff, where return is measured by the expectation of the reward and risk is measured by variance. However, they usually focus on selecting single arm, with goals to maximize return, there is a lack of work on combinatorial setting where the goal is to get close to a target. 

%There have been works on MAB algorithm design for reducing and controlling risks (cite??). However, most papers consider selecting 


% of monotonicity or the uniqueness of the optimal solution required in \citep{chen2016combinatorial}. 

%They propose the Combinatorial Upper Confidence Bound (CUCB) using the principle of \textit{optimism in the face of uncertainty}. \textcolor{red}{Another line of work follows the \textit{Bayesian} approach and studys Thompson sampling \citep{gopalan2014thompson} \citep{wang2018thompson}. However, the regret bounds of Thompson sampling depend  exponentially on the number of the selected arms $K$ and  \citep{wang2018thompson} shows that the exponential dependence is unavoidable.}




%\textcolor{red}{The reliability objective of our CMAB problem does not satisfy the conditions of monotonicity or the uniqueness of the optimal solution required in \citep{chen2016combinatorial}. Moreover, in practice, $K$ is large because we aim to select a large number of customers to ensure reliability, thus Thompson sampling may generate poor performance. Therefore, either the learning algorithms or the analysis in literature does not suit our CMAB problem, motivating us to design new CMAB algorithms.}

%However, our CMAB problem with the reliability objective function does not satisfy the conditions of monotonicity or the uniqueness of the optimal solution, and a properly selected prior distribution for our problem may not satisfy the assumption in \citep{gopalan2014thompson}.
%Therefore,  either the  learning approaches or the analysis  in current literature do not suit our CMAB problem, motivating us to design new CMAB algorithms.

\textit{Preliminary work.} Some preliminary work was presented in the conference paper \citep{li2018learning}. This journal version strengthens the regret bounds, especially for the time-varying  target case, conducts  more intensive numerical analysis using realistic data from ISOs, provides more complete proofs, and adds more  intuitions and discussions to both theoretical and numerical results.



%\textit{Organization of the Paper.} Section II introduces the problem formulation. Section III introduces an offline algorithm and an online algorithm CUCB-Avg. Section IV studies the performance guarantee for a time-invariant target. Section V studies the performance guarantee for a time-varying target. Section VI provides the simulation results. 

\vspace{6pt}
\noindent\textbf{Notations.} Let $\bar E$ and $|E|$ be the complement and the cardinality of the set $E$ respectively. For any positive integer $n$, let $[n]=\{1,\dots, n \}$. Let $I_E(x)$ be the indicator function: $I_E(x)=1$ if $x\in E$ and $I_E(x)=0$ if $x\not \in E$. For any two sets $A, B$, we define $A-B\coloneqq\{x\mid x\in A, x\not \in B \}$. When $k=0$, let $\sum_{i=1}^k a_i=0$ for any $a_i$, and define the set $\{\sigma(1),\dots, \sigma(k) \}=\emptyset$ for any $\sigma(i)$. %Finally, we define the big-O and small-o notations.
 For $x\in \R^k$,  we consider $\|x\|_\infty = \max_{i\in[k]}|x_i|$, and
 write $f(x)=O(g(x))$ as $\|x\|_\infty \to +\infty$  if there exists a constant $M$ such that $|f(x) | \leq M |g(x)|$ for any $x$ with $x_i\geq M$ for some $i$; and  $f(x)=o(g(x))$  if $ f(x)/g(x)\to0$ as $\|x\|_\infty \to +\infty$. We usually omit ``as $\|x\|_\infty\to +\infty$" for simplicity. For the asymptotic behavior near zero,  consider the inverse of $\|x\|_\infty$. 







==> arxiv submit/sec2_problem_formulation.tex <==
\section{Problem Formulation}



Motivated by the discussion above, we formulate the demand response (DR)  as a CMAB problem in this section. We  focus on load reduction to illustrate the problem. The load increase can be treated in the same way. 

%We consider a DR program in $T$ time steps, where each time step corresponds to one DR event.\footnote{The specific definition of DR events and the duration of each event is up to the choice of the system designer. Our methods can accommodate different scenarios.} There is one aggregator and $n$ residential customers in the DR program. 



Consider a DR program with an aggregator and $n$ residential customers  over $T$ time steps, where each time step corresponds to one DR event.\footnote{The specific definition of DR events and the duration of each event are up to the choice of the system designer. Our methods can accommodate different scenarios.} Each customer is viewed as an arm in our CMAB problem. We consider a simple user (customer) behavior model, where each customer may either respond to a DR event by reducing one unit of power consumption with probability $0\leq p_i\leq 1$, or not respond with probability $1-p_i$. We denote the demand reduction by customer $i$ at time step $t$ as $X_{t,i}$, which is assumed to follow Bernoulli distribution, $X_{t,i}\sim \text{Bern}(p_i)$, and is independent across time.\footnote{For simplicity, we only consider that each customer has one unit to reduce. Our learning method can be extended to multi-unit setting and/or the setting where different users have different sizes of units. But the regret analysis will be more complicated which we leave as future work. As mentioned before, results in the paper have been used as a guideline for DR field studies \citep{conEdison}.} Different customers behave independently and may respond to the same DR event with  different probabilities. Though this behavior model may be oversimplified by neglecting the influences of temperatures, humidities, user fatigue, changes in lifestyles, etc., this simple model allows us to provide useful insights on improving the  reliability of the DR programs and lay the foundation for future  research on more realistic behavior models.



%We will call each customer as an arm. consider a simple user behavior model


 %Each customer is viewed as an arm in CMAB. This paper considers a simplified customer behavior model where each customer may respond to a DR event by reducing one unit of power consumption with probability $0\leq p_i\leq 1$, or not respond with probability $1-p_i$. 
%The demand reduction by customer $i$ at time step $t$ is denoted by $X_{t,i}$, which is assumed to follow Bernoulli distribution: $X_{t,i}\sim \text{Bern}(p_i)$ and is independent across time.\footnote{For simplicity, we only consider that each customer has one unit to reduce. Our learning method can be extended to multi-unit setting and/or the setting where different users have different size of units. But the regret analysis will be more complicated which we leave as future work. As mentioned before, results in the paper have been used as a guideline for DR field studies\citep{conEdison}.} Different customers respond to the DR events  with possibly different probabilities independently.  Though the behavior model may be oversimplified by neglecting the influences of temperatures, humidities, user fatigue, changes in lifestyles, etc., this simple model allows us to provide useful insights into how to improve the reliability of the DR programs and lay the foundation for future  research on more realistic behavior models.

%obtain interesting design and analysis for reliability and provide insights and foundation for research on more realistic behavior models.

%described above is simplified and does not capture the effects of user fatigue, temperature, humidity, etc, but this simple model enables us to conduct 

 %Nevertheless, the algorithm design and analysis for reliability concerns built on this simple model can serve as foundation for future work that considers more realistic models.



At each time $1\leq t\leq T$, there is a DR event with a nonnegative demand reduction target $D_t$ determined by the power system. This reduction target might be caused by a sudden drop of renewable energy generation or a peak load reduction request, etc. 
The aggregator aims to select a subset of customers, i.e. $S_t \subseteq [n]$, such that the total demand reduction is as close to the target as possible. The cost at time $t$ can be captured by the \textit{squared deviation} of the total reduction from the target $D_t$: 
$$ L_t(S_t)= \left(\sum_{i\in S_t}X_{t,i}-D_t\right)^2.$$
Noticing that the  demand reduction $X_{t,i}$ are random, we consider a goal of selecting a subset of customers $S_t$ to minimize the   squared deviation in expectation, that is,
\begin{equation}\label{equ: problem formulation}
S_t^* \subseteq \argmin_{S_t \subseteq [n]} \E\!\left[ L_t(S_t)\right].
\end{equation}
	In this paper, we will first study the scenario where the target $D$ is time-invariant (Section~\ref{sec: online alg} and \ref{sec: regret}). Then, we will extend the results to cope with time-varying targets to
	incorporate different DR signals resulted from the fluctuations of power supply and demand (Section~\ref{sec:time_varying}). 

When the response probability profile $ p=(p_1, \dots, p_n)$ is known, the problem \eqref{equ: problem formulation} is a combinatorial optimization. In Section \ref{sec: online alg}, we will provide an offline combinatorial optimization algorithm to solve the problem \eqref{equ: problem formulation}.

In reality, the response  probabilities are usually unknown. Thus, the aggregator should learn the probabilities from the feedback of the previous demand response events, then make online decisions to minimize the difference between the total demand reduction and the target $D_t$. The learning performance is measured by $\text{Regret}(T)$, which compares the total expected cost of online decisions and the optimal total expected costs in $T$ time steps:\footnote{Strictly speaking, this is the definition of pseudo-regret, because its benchmark is the optimal expected cost: $\min_{S_t \subseteq [n]}\E L_t(S_t) $, instead of the optimal cost for each time, i.e. $\min_{S_t \subseteq [n]} L_t(S_t) $.}
\begin{equation}
\begin{aligned}
&\text{Regret}(T) \coloneqq \E\left[\sum_{t=1}^T R_t(S_t)\right], \label{equ:regret def}
\end{aligned} 
\end{equation}
where $ R_t(S_t)\coloneqq L_t(S_t) - L_t(S^*_t)$ and the expectation is taken with respect to  $X_{t,i}$ and the possibly random $S_t$.


The feedback of previous demand response events includes the responses of every selected customer, i.e., $\{X_{t,i}\}_{i\in S_t}$. Such feedback structure is called \textit{semi-bandit} in literature \citep{chen2016combinatorial}, and carries more information than bandit feedback which only includes the realized cost $L_t(S_t)$.














Lastly, we note that our problem formulation can be applied to other applications beyond demand response. One example is introduced below.



\begin{example}
	Consider a crowd-sourcing related problem. Given  budget $D_t$, a survey planner sends out surveys and offers one unit of reward for each participant. Each potential participant may  participate with probability $p_i$. Let $X_{t,i}=1$ if agent $i$ participates; and $X_{t,i}=0$ if agent $i$ ignores the survey. The survey planner intends to maximize the total number of responses without exceeding the budget too much. One possible formulation 
	 is to select subset $S_t$ such that the total number of responses is close to the budget $D_t$, 
	 $$ \min_{S_t} \E\left(\sum_{i\in S_t}X_{t,i}-D_t\right)^2.$$
	 Since the participation probabilities are unknown, the  planner can learn the participation probabilities from the previous actions of the selected agents and then try to minimize the total costs during the learning process. 
\end{example}




==> arxiv submit/sec3_algorithm.tex <==
\section{Algorithm Design} \label{sec: online alg}
This section considers time-invariant target $D$. We will first  provide an optimization algorithm for the offline problem, then introduce the notations for online algorithms and discuss two simple algorithms: greedy algorithm and CUCB. Finally, we introduce our online algorithm CUCB-Avg. % and provide intuitions behind the algorithm design.
\subsection{Offline Optimization}
When the probability profile $p$ is known, the problem \eqref{equ: problem formulation} becomes a combinatorial optimization problem:
\begin{align}\label{equ: offline minimization}
\min_{S \subseteq [n]} \left[(\sum_{i\in S}p_i-D)^2+ \sum_{i\in S}p_i(1-p_i)\right],
\end{align}
where we omit the subscript $t$ for simplicity of notation.
Though combinatorial optimization is NP-hard  and only has approximate algorithms in general, we are able to design a simple algorithm in Algorithm \ref{alg: offline oracle} to solve the problem \eqref{equ: offline minimization} exactly. Roughly speaking, Algorithm \ref{alg: offline oracle} takes two steps: i) rank the arms according to $p_i$, ii) determine the number $k$ according to the probability profile $p$ and the target $D$ and select the top $k$ arms. The output of Algorithm~\ref{alg: offline oracle} is denoted by $\phi(p,D)$ which is a subset of $[n]$. In the following theorem, we show that such algorithm finds an optimal solution to  \eqref{equ: offline minimization}. 

\begin{algorithm}\caption{Offline optimization algorithm}\label{alg: offline oracle}
	\begin{algorithmic}[1]
		\State \textbf{Inputs:}  $p_1,\dots,  p_n\in [0,1]$, $D>0$.
		\State Rank $p_i$ in a non-increasing order: 
		
		
		$ p_{\sigma(1)}\geq \dots \geq p_{\sigma(n)}$.
		\State Find the smallest $k\geq 0$ such that
$$
		\sum_{i=1}^k p_{\sigma(i)}> D-1/2.$$
Let $k=n$ if
$
		 \sum_{i=1}^{n} p_{\sigma(i)}\leq D-1/2
$. Ties are broken randomly.
		\State \textbf{Ouputs}:  $\phi(p,D)=\{\sigma(1),\dots, \sigma(k) \}$
	\end{algorithmic}
\end{algorithm}
\begin{theorem}\label{thm: offline opt optimality}
	For any $D>0$, the output of
	Algorithm \ref{alg: offline oracle}, $\phi(p, D)$, is an optimal solution to \eqref{equ: offline minimization}.
\end{theorem}
\textit{Proof Sketch.}
We defer the detailed proof to Appendix \ref{aped: offline opt} and only introduce the intuition here. An optimal set $S$  roughly has two properties: i) the total expected contribution of $S$, $\sum_{i\in S} p_i$, is closed to the target $D$, ii) the total variance of  arms in $S$ is minimized. i) is roughly guaranteed by Line 3 of Algorithm \ref{alg: offline oracle}: it is easy to show that $|\sum_{i\in\phi(p,D)} p_i-D|\leq 1/2$. ii) is roughly guaranteed by only selecting arms with higher response probabilities, as indicated by Line 2 of Algorithm \ref{alg: offline oracle}. The intuition is the following. Consider an arm with large parameter $p_1$ and two arms with smaller parameters $p_2, p_3$. For simplicity, we let $p_1=p_2+p_3$. Thus replacing $p_1 $ with $p_2,p_3$ will not affect the first term in \eqref{equ: offline minimization}. However, 
$ p_1(1-p_1) \leq p_2(1-p_2) + p_3(1-p_3)$
by $p_1^2=(p_2+p_3)^2 \geq p_2^2+p_3^2$.
Hence, replacing one arm with higher response probability by two arms with lower response probabilities will  increase the variance. 
\qed

\begin{corollary}\label{cor: D<1/2}
	When $D<1/2$, the empty set is optimal. 
\end{corollary}
\begin{remark}
	There might be more than one optimal subset. Algorithm \ref{alg: offline oracle} only outputs one of them.
\end{remark}



\subsection{Notations for Online Algorithms}

Let $\bar p_i(t)$ denote the sample average of parameter $p_i$ by time $t$ (including time $t$), then 
$$ \bar p_i(t) = \frac{1}{T_i(t)}\sum_{\tau \in I_i(t)} X_{\tau, i},$$
where  $I_i(t)$ denotes the set of time steps when arm $i$ is selected by time $t$ and $T_i(t)=| I_i(t)| $ denotes the number of times that arm $i$ has been selected by time $t$. 
Let $\bar p(t) = (\bar p_1(t), \dots, \bar p_n(t))$.
Notice that before making decisions at time $t$, only $\bar p(t-1)$ is available.

\subsection{Two Simple Online Algorithms: Greedy Algorithm and CUCB}\label{subsec: CUCB}
Next, we introduce two simple methods: greedy algorithm and CUCB, and explain their poor performance in our problem to gain intuitions for our algorithm design.


Greedy algorithm  uses the sample average of each parameter $\bar p_i(t-1)$ as an estimation of the unknown probability $p_i$ and chooses a subset based on the offline oracle described in Algorithm~\ref{alg: offline oracle}, i.e. $S_t = \phi(\bar p(t-1),D)$. The greedy algorithm is known to perform poorly  because  it
only exploits the current information, but fails to explore the unknown information, as demonstrated below. 
\begin{example}
Consider two arms that generate Bernoulli rewards with  expectation $p_1>p_2>0$. The goal is to select the arm with the higher  reward expectation, which is arm 1 in this case. Suppose after some time steps, arm 1's history sample  average $\bar p_1(t)$ is zero, while arm 2's history average $\bar p_2(t)$ is positive. In this case, the greedy algorithm will always select the suboptimal arm 2 in the future since $\bar p_2(t)>\bar p_1(t)=0$ for all future time $t$ and arm 1's history average will remain 0 due to insufficient exploration. Hence, the regret will be $O(T)$.
	
	
%	If we apply greedy algorithm, we will continue to select arm 2 since arm 2's history sample average $\bar p_2(t)$ is positive while arm 1's history average $\bar p_1(t)=0$. As a result, the greedy algorithm will always select the suboptimal arm and generate $O(T)$ regret.
	
	
	% and thus always larger than $\bar p_1(t)=0$, 
	
	
%	which is the  after some time steps, we have explored the suboptimal arm 2 for enough times such that  $\bar p_2 \approx p_2$, but haven't explored the optimal arm 1 enough so that $\bar p_1$ is an underestimate and satisfies: $\bar p_1 < \bar p_2 <p_1$. In this case, the greedy algorithm will keep selecting the suboptimal arm 2 based on current estimation $\bar p_1, \bar p_2$ and fail to explore arm 1. As a result, the regret will be $O(T)$. 
\end{example}


A well-known algorithm in CMAB literature  that balances the exploration and exploitation is CUCB \citep{chen2016combinatorial}. Instead of using sample average $\bar p(t-1)$ directly, CUCB considers an upper confidence bound:
\begin{equation} \label{eq:Ui}
	 U_i(t) =\min\left( \bar p_i(t-1)+ \sqrt{\frac{\alpha \log t}{2T_i(t-1)}},1\right),
\end{equation}
{\color{black}
where $\alpha\geq 0$ is the parameter to balance the tradeoff between $\bar p_i(t-1)$ (exploitation) and $T_i(t-1)$ (exploration). The output of CUCB is $S_t= \phi(U(t), D)$.  CUCB performs well in classic CMAB problems, such as maximizing the total contribution of $K$ arms for a fixed  $K$.

%for the exploration-exploitation tradeoff. Then CUCB applies the offline oracle
%$S_t= \phi(U(t), D)$ where $U(t) = (U_1(t), \dots, U_n(t))$. $U_i(t)$ is restricted to $[0,1]$ in case $U(t)$ is outside the domain of the oracle $\phi$. $U_i(t)$ is also known as the upper confidence bound of $p_i$, and is restricted to $[0,1]$  allows the algorithm to balance exploration and exploitation, because it carries the information of both the sample average, and the number of exploration times $T_i(t-1)$.
% CUCB performs well in classic CMAB problems, such as maximizing the total contribution of $K$ arms for a fixed number $K$ \citep{kveton2015tight,chen2016combinatorial}. 

% CUCB selects arms with high upper confidence bounds $U_i(t)$. 

% CUCB  well in classic combinatorial multi-armed bandit problems, such as selecting the top $K$ arms. The intuition is the following. CUCB tends to select arms with higher upper confidence bounds $U_i(t)$. There are two cases in which $U_i(t)$ is large, first, the sample average is large, second, $T_i(t)$ is small, indicating arm $i$ is underexplored. Therefore, CUCB selects both arms with higher sample average, and also under-explored arms.


However, CUCB performs poorly in our problem, as shown in Section \ref{sec: simulation}. }The major problem of CUCB is the over-estimate of the arm parameter $p$. By choosing $S_t= \phi(U(t), D)$, CUCB selects less arms than needed, which not only results in a large deviation from the target, but also discourages exploration.


% I don't know how to create footnote in algorithm environment
\begin{algorithm}\caption{CUCB-Avg}\label{alg: ucb_avg}
	\begin{algorithmic}[1]
		\State \textbf{Notations:}  $T_i(t)$ is the number of times selecting 
		arm $i$ by  time  $t$, and $\bar p_i(t)$ is the sample average of  arm $i$ by time $t$ (both including time $t$).
		\State \textbf{Inputs:} $\alpha$, $D$.
		\State \textbf{Initialization:}  For $t=1, \ldots, \ceil{\frac{n}{\ceil{2D}}}$, select $\ceil{2D}$ arms each time until each arm has been selected for at least once.
			Let $S_t$ be the set of arms selected at time $t$. Initialize $T_i(t)$ and $\bar p_i(t)$ by the observation $\{X_{t,i} \}_{i\in S_t}$.\textcolor{black}{\footnotemark{}}
			%\textcolor{red}{add a couple of sentences as a footnote explaining why do this initialization and pointing out that this initialization is non-unique and flexible. I tried to add a footnote but the footnote couldn't be shown if it is added inside the algorithm...}} 
		\For{$t=\ceil{\frac{n}{\ceil{2D}}}+1, \dots, T$ }
		\State 	Compute the upper confidence bound for each  $i$
		
		$U_i(t) = \min\left( \bar p_i(t-1)+ \sqrt{\frac{\alpha \log t}{2T_i(t-1)}},1\right)$.
		
		\State 	Rank $U_i(t)$ by a non-increasing order:  
		
		$U_{\sigma(t,1)}(t)\geq \dots \geq U_{\sigma(t,n)}(t)$.
		\State Find the smallest $k_t\geq 0$ such that 
		$$ \sum_{i=1}^{k_t} \bar p_{\sigma(t,i)}(t-1)>D-1/2$$
		\qquad or let $k_t=n$ if $ \sum_{i=1}^{n} \bar p_{\sigma(t,i)}(t-1)\leq D-1/2$. 
		\State  Select $S_t=\{\sigma(t,1),\dots, \sigma(t, k_t) \}$ 
		\State Update $T_i(t)$ and $\bar p_i(t)$ by observations $\{X_{t,i} \}_{i\in S_t}$
		\EndFor
	\end{algorithmic}
\end{algorithm}\footnotetext{\textcolor{black}{The initialization method  is
not unique and can be any method that selects each customer
for at least once.}}





\subsection{Our Proposed Online  Algorithm: CUCB-Avg}
Based on the discussion above, we propose a new method CUCB-Avg. The novelty of CUCB-Avg is that it utilizes both sample averages and upper confidence bounds by exploiting the structure of the offline optimal method. 

We note that the offline Algorithm~\ref{alg: offline oracle} selects the right subset of arms in two steps: i)  rank (top) arms, ii) determine the number $k$ of the top arms to select. In CUCB-Avg, we use the upper confidence bound $U_i(t)$ to rank the arms in a non-increasing order. This is the same as  CUCB. However, the difference is that our CUCB-Avg uses the sample average $\bar{p}_i(t-1)$ to decide the number of  arms to select at time $t$. The details of the algorithm are given in Algorithm~\ref{alg: ucb_avg}.

Now we explain  why the ranking rule and the selection rule of CUCB-Ave would work for our problem. 

The ranking rule is determined by $U_i(t)$. An arm with larger $U_i(t)$ is given a priority to be selected at time $t$. We note that  $U_i(t)$ is the summation of two terms: the sample average $\bar{p}_i(t-1)$ and the confidence interval radius that is related to how many times the arm has been explored. Therefore, an arm with a large $U_i(t)$ may    have a small $T_i(t-1)$, meaning  that the arm has not been explored enough; and/or  have a large $\bar p_i(t-1)$, indicating that the arm frequently responds in the history. In this way, CUCB-Avg selects both the under-explored arms (\textit{exploration}) and the arms with good performance in the past (\textit{exploitation}). 

 
 
When determining $k$, CUCB-Avg uses the sample averages and selects enough arms such that the total sample average is close to $D$. Compared with CUCB which uses upper confidence bounds to determine $k$, our algorithm selects more arms, which reduces the load reduction difference from the target and also encourages  exploration.

%\textcolor{red}{Finally, we note that the initialization method (Line 3) is not unique and can be any method that selects each customer for at least once in the first several time steps.   


==> arxiv submit/sec4_regret.tex <==
\vspace{-8pt}

\section{Regret analysis}\label{sec: regret}
In this section, we will prove that our algorithm CUCB-Avg achieves $O(\log T)$ regret when $D$ is time invariant.

\subsection{The Main Result}
%The next theorem upper bounds the regret of CUCB-Avg. 

\begin{theorem}\label{thm: regret bdd D}
	%Consider  $n$ arms with parameter $p=(p_1,\dots, p_n)$ over $T$ time steps. 
	There exists a constant $\epsilon_0>0$ determined by $p$ and $  D$, such that 
	for any $\alpha>2$, the regret of CUCB-Avg is upper bounded by
	\begin{equation}\label{equ: regret bdd D}
	\textup{Regret}(T)\leq M\left(\ceil{\frac{n}{\ceil{2D}}}+\frac{2 n}{\alpha -2}\right)+ \frac{\alpha Mn\log T}{2\epsilon_0^2}, 
	\end{equation}
	where $M=\max(D^2, (n-D)^2)$. 
\qed	
\end{theorem}

We make a few comments before the proof.

{\color{black}
%\vspace{4pt}
\nbf{Dependence on  $T$ and $n$.} The  dependence on the horizon $T$ is $O(\log T)$, so the average regret diminishes to zero as $T$ increases, indicating that our algorithm learns the customers' response probabilities effectively. The dependence on $n$ is polynomial, i.e. $O(n^3)$ by $M\sim O(n^2)$, showing that our algorithm  can handle a large number of arms effectively. The cubic dependence is likely to be a proof artifact and improving the dependence on $n$ is left as future work.

%The dependence on the number of arms $n$ is polynomial, demonstrating that CUCB-Avg can handle a large number of arms. Since $M=O(n^2)$,$O(n^3)$. The polynomial dependence demonstrates that our algorithm can handle a large number of arms. The cubic dependence on $n$ might be a proof artifact and is left to be improved in future work. %improving the dimension dependence is left for future work. %The bound also depends on a constant term $\epsilon_0$ determined by $p$ and $D$ and such a bound is  referred as a \textit{distribution-dependent  bound} in literature.  % as $p$ is invariant with horizon $T$ \citep{bubeck2012regret}. 

%eading term in the regret bound \eqref{equ: regret bdd D} is  $O(n^3\log T/\epsilon_0^2)$ since $M \sim O(n^2)$ and $\epsilon_0$ is a constant determined by $p$ and $D$. Besides, the constant term is $O(n^3)$, which is polynomial on the number of arms. %When compared with the regret bound for Thompson sampling \citep{wang2018thompson}, our regret bound is 
%The bound is referred as a \textit{distribution-dependent  bound} in literature as $p$ is invariant with horizon $T$ \citep{bubeck2012regret}. 
}


%\textcolor{red}{Require poly on $K$ by refine $M$'s def.}

%\vspace{4pt}

%$\alpha$ shows up in two terms: $\frac{2M n}{\alpha -2}$ and $ \frac{\alpha Mn\log T}{2\epsilon_0^2} $.  The first term grows when $\alpha$ decreases, and the second one decreases when $\alpha$ decreases. Since the second term is $O(\log T)$ while the first term is constant with respect to $T$, $\alpha$ should be chosen to be close to $2$ when $T$ is large. 

%\vspace{4pt}
{\color{black}
\nbf{Role of $\epsilon_0$.} The bound depends on a constant term $\epsilon_0$ determined by $p$ and $D$ and such a bound is  referred to as a \textit{distribution-dependent  bound} in literature. We defer the explicit expression of $\epsilon_0$ to Appendix \ref{aped: D no regret} and only explain the intuition behind $\epsilon_0$ here. Roughly, $\epsilon_0$ is a robustness measure of our offline optimal algorithm, in the sense that  if the probability profile $p$ is perturbed  by $\epsilon_0$, i.e., $ |\tilde p_i-p_i|< \epsilon_0$ for all $i$, the output $\phi(\tilde p,D)$ of Algorithm~\ref{alg: offline oracle} would still be  optimal for the true profile $p$. Intuitively, if $\epsilon_0$ is large, the learning task is easy because we are able to find an optimal subset given a poor estimation, leading to a small regret. This explains why the upper bound in (\ref{equ: regret bdd D}) decreases when $\epsilon_0$ increases.
}

%To start with, we explain why the upper bound in (\ref{equ: regret bdd D}) decreases when $\epsilon_0$ increases. Roughly speaking, $\epsilon_0$ is a robustness measure of our offline optimal algorithm, in the sense that  if the probability profile $p$ is perturbed to be $\bar p$ by $\epsilon_0$ (i.e., $ |\bar p_i-p_i|< \epsilon_0$ for all $i$), Algorithm~\ref{alg: offline oracle}'s output $\phi(\bar p,D)$ would still be  optimal for the true profile $p$. Intuitively, if $\epsilon_0$ is large, the learning task is easy because we are able to find an optimal subset given a poor estimation, leading to a small regret.


To discuss what factors will affect the robustness measure $\epsilon_0$, we provide an explicit expression of $\epsilon_0$ under two assumptions in the following proposition.

\begin{proposition}\label{prop: A1A2 epsilon0}
	Consider the following  assumptions.\\
	\textup{(A1)} 	$p_i$ are positive and distinct $p_{\sigma(1)}> \dots > p_{\sigma(n)}>0$. \\
	\textup{(A2)}	There exists $k\geq 1$ such that 
	$ \sum_{i=1}^k p_{\sigma(i)}> D-1/2,$ and $ \sum_{i=1}^{k-1} p_{\sigma(i)}< D-1/2
$.\\
	Then the $\epsilon_0$ in Theorem \ref{thm: regret bdd D} can be determined by:
	\begin{equation}
	\epsilon_0 = 
	\min\left(\frac{\delta_1}{k}, \frac{\delta_2}{k}, \frac{\Delta_k}{2}\right),
	\label{equ: def epsilon}
	\end{equation}
	where $k=| \phi(p, D)|$, $\sum_{i=1}^k p_{\sigma(i)}=D-1/2+\delta_1,$ $ \sum_{i=1}^{k-1} p_{\sigma(i)}=D-1/2-\delta_2,$ and $\Delta_i =p_{\sigma(i)}-p_{\sigma(i+1)} ,  \forall \ i=1,\dots, n-1$.
%	\begin{equation}\label{equ: def delta}
%	\begin{aligned}
%	& k=| \phi(p, D)|\\
%	& \sum_{i=1}^k p_{\sigma(i)}=D-1/2+\delta_1, \\
%	& \sum_{i=1}^{k-1} p_{\sigma(i)}=D-1/2-\delta_2,\\
%	& \Delta_i =p_{\sigma(i)}-p_{\sigma(i+1)} ,  \forall \ i=1,\dots, n-1
%	\end{aligned}
%	\end{equation}	
\end{proposition}
We defer the proof of the proposition to Appendix \ref{aped: D no regret Ass} and only make two comments here. Firstly, it is easy to verify that Assumptions (A1) and (A2) imply $\epsilon_0>0$. Secondly, we explain why $\epsilon_0$ defined in \eqref{equ: def epsilon} is a robustness measure, that is, we show if $\forall\, i,\ | \tilde p_i- p_i| <\epsilon_0$,  then $\phi(\tilde p, D)=\phi(p,D)$. This can be proved in two steps. Step 1: when $\epsilon_0 \leq \frac{\Delta_k}{2}$,
the $k$ arms with higher $\tilde {p}_i$ are the same $k$ arms with higher $p_i$ because for any $1\leq i \leq k$ and $k+1 \leq j \leq n$, we have $
\tilde p_{\sigma(i)}> p_{\sigma(k)}-\epsilon_0 \geq p_{\sigma(k+1)} + \epsilon_0> \tilde p_{\sigma(j)}$. 
 Step 2: by $\epsilon_0 \leq \min\left( \frac{\delta_1}{k},\frac{\delta_2}{k}\right)$ and the definition of $\delta_1$ and $\delta_2$, when $|\tilde p_i-p_i|\leq \epsilon_0$ for all $i$,  we have $\sum_{i=1}^k \tilde p_{\sigma(i)}> D-1/2$ and $\sum_{i=1}^{k-1} \tilde p_{\sigma(i)}  < D-1/2$. Consequently, by Algorithm \ref{alg: offline oracle}, $\phi(\tilde p, D)=\{\sigma(1),\dots, \sigma(k) \}=\phi(p,D)$.


Finally, we briefly discuss how to generalize the expression \eqref{equ: def epsilon} of $\epsilon_0$ to cases without (A1) and (A2). When (A1) does not hold, we only consider the gap between the arms that are not in a tie, i.e. $\{\Delta_i| \ \Delta_i>0, \  1\leq i\leq n-1 \}$. When (A2) does not hold and $\sum_{i=1}^{k-1} p_{\sigma(i)}=D-1/2$, we consider  less than $k-1$ arms to make the total expected contribution below $D-1/2$. An explicit expression of $\epsilon_0$ is provided in Appendix \ref{aped: D no regret}.

{\color{black}
\nbf{Comparison with the regret bound of classic CMAB.}
In classic CMAB literature when the goal is to select $K$ arms with the highest parameters given a fixed integer $K$, the regret bound usually depends on $\frac{\Delta_K}{2}$ \citep{kveton2015tight}. We note that $\frac{\Delta_K}{2}$ is similar to  $\epsilon_0$ in our problem, as it is the robustness measure of the top-$K$-arm problem in the sense that given any estimation $\tilde p$ with estimation error at most $\frac{\Delta_K}{2}$: $\forall\, i,\ | \tilde p_i- p_i| <\frac{\Delta_K}{2}$,  the top $K$ arms with the profile $\tilde p$ are the same as that with the profile $p$. In addition, we would like to mention that the regret bound in literature is usually linear on $1/\Delta_K$, while our regret bound is $1/\epsilon_0^2$. This difference may be an artificial effect of the proof techniques because our CMAB problem is more complicated. We leave it as future work to strengthen the results. 
}
%In addition, the regret bound in literature is $O(\frac{\log T}{\Delta_K/2})$ as $\Delta_K $ goes to zero \citep{kveton2015tight}, while our regret bound in \eqref{equ: regret bdd D} is $O(\frac{\log T}{\epsilon_0^2})$. This difference on the dependence on the  may be due to technical reasons.



%\nbf{Choice of $\alpha$.} When $\alpha $ increases, the term $\frac{2M n}{\alpha -2}$ decreases while the term $ \frac{\alpha Mn\log T}{2\epsilon_0^2} $ increases. Since the second term is $O(\log T)$ while the first term is $O(1)$, $\alpha$ should be  close to $2$ when $T$ is large. 


%\vspace{6pt}


\subsection{Proof of Theorem \ref{thm: regret bdd D}}
%\textcolor{red}{D<=1/2, some claim also breaks.}


\nbf{Proof outline:} We divide the $T$ time steps into four parts, and bound the regret in each part separately. The partition of the time steps are  based on event $E_t$ and the event $B_t(\epsilon_0)$ defined below.
Let $E_t$ be the event when the sample average is outside the confidence interval considered in Algorithm \ref{alg: ucb_avg}: 
$$ E_t \coloneqq \left\{ \exists \, i\in [n], \ |\bar p_i(t-1) -p_i|\geq \sqrt{\frac{\alpha \log t}{2 T_i(t-1)}}   \right\}.$$
For any $\epsilon>0$, let $B_t(\epsilon)$ denote the event when Algorithm \ref{alg: ucb_avg} selects an arm who has been explored for no more than $ \frac{\alpha \log T}{2\epsilon^2} $ times:
\begin{equation}
B_t(\epsilon)\coloneqq \left\{ \exists \, i\in S_t, \ s.t. \ T_i(t-1) \leq \frac{\alpha \log T}{2\epsilon^2}   \right\}. \label{eq:Btepsilon}
\end{equation} 
Let $\epsilon_0>0$ be a  small number  such that Lemma \ref{lem: no regret bar E bar B} holds.

Now, we will define the four parts of the $T$ time steps, and briefly introduce the regret bound of each part. 


\begin{enumerate}%[\leftmargin=5pt]
	\item \textit{Initialization:} the regret bound does not depend on $T$ (Inequality (\ref{eq: D Rt(St)<= M})).
	\item \textit{When event $E_t$ happens:} the regret  bound does not depend on $T$ because $E_t$ happens rarely due to concentration properties in statistics (Lemma \ref{lem: regret 1bdd}).
	\item \textit{When event $\bar E_t$ and $B_t(\epsilon_0) $ happen:} the regret is at most $O(\log T)$ because $B_t(\epsilon_0)$ happens for at most $O(\log T)$ times (Lemma \ref{lem: regret4 bdd}).
	\item \textit{When  event $\bar E_t$ and $\bar B_t(\epsilon_0) $ happen,} the regret is zero due to the  enough exploration of the selected arms (Lemma \ref{lem: no regret bar E bar B}).
\end{enumerate}
Notice that the time steps are not divided sequentially here. For example, it is possible that $t=10$ and $t=30$ belong to Part 2 while $t=10$ belongs to Part 3.

%\vspace{6pt}
\nbf{Proof details:} Firstly, it is without loss of generality to require $D\geq 1/2$ because when $D<1/2$, the optimal set is known to be the empty set by Corollary \ref{cor: D<1/2}, so the regret is zero by selecting no customers.

Secondly, we note that for all time steps $1\leq t\leq T$ and any $S_t\subseteq[n]$, the regret at   $t$ is upper bounded by 
\begin{align}
R_t(S_t )&  \leq L_t(S_t)      \leq  \max(D^2, (n-D)^2)  \eqqcolon M. \label{eq: D Rt(St)<= M}
\end{align}
% note: n cannot be replaced by sum_i p_i. We need bound on realized Rt, not expected Rt
Thus, the regret of initialization (Part 1) at $t=1,\dots, \ceil{\frac{n}{\ceil{2D}}}$ is  bounded by $M\ceil{\frac{n}{\ceil{2D}}}$.


Next, we bound the regret of Part 2 by the  Chernoff-Hoeffding's concentration  inequality. The intuition behind the proof is that $E_t$ happens rarely because the sample average $\bar{p}_i(t)$ concentrates around the true value $p_i$ with a high probability. 
\begin{theorem}[Chernoff-Hoeffding's inequality]\label{thm: chernoff}
Consider i.i.d. random variables $X_1,\dots, X_m$ with support  $[0,1]$ and mean $\mu$, then we have
	\begin{equation}
	\Pb\left(|\sum_{i=1}^m X_i -m\mu |\geq m \epsilon\right)\leq 2 e^{-2m \epsilon^2} .
	\end{equation}
\end{theorem}


\begin{lemma}\label{lem: regret 1bdd}
	
	When $\alpha>2$, we have
$$
	\E \left[\sum_{t=1}^T I_{E_t} R_t(S_t)\right]\leq \frac{2Mn}{\alpha -2}.
$$
\end{lemma}
%\nit{Proof.}
\begin{proof} The number of times $E_t$ happens is bounded by
%	By Inequality \eqref{eq: D Rt(St)<= M} and the fact $I_{E_t}\geq 0$, we have,
%	\begin{align*}
%	&\E \sum_{t=1}^T I_{E_t} R_t(S_t)\leq M \E \sum_{t=1}^T I_{E_t} .
%	\end{align*}
%	So we only need to bound $\E \sum_{t=1}^T I_{E_t} $.
	\begin{align*}
	&	\E \left[\sum_{t=1}^T I_{E_t} \right]= \sum_{t=1}^T \Pb(E_t)   \\
	& \leq \sum_{t=1}^T \sum_{i=1}^n  \Pb\left(|\bar p_i(t-1)-p_i| \geq \sqrt{\frac{\alpha \log t}{2 T_i(t-1)}}\right)   \\
	& \leq \sum_{t=1}^T \sum_{i=1}^n  \sum_{s=1}^{t-1}\Pb(|\bar p_i(t-1)-p_i| \geq \sqrt{\frac{\alpha \log t}{2 s}},  T_i(t-1)  = s)   \\
	& \leq \sum_{t=1}^T \sum_{i=1}^n  \sum_{s=1}^{t-1}\, \frac{2}{t^\alpha}  \leq \sum_{t=1}^T \, \frac{2n}{t^{\alpha-1}}   \leq \frac{2n}{\alpha -2},
	\end{align*}
	where the first inequality is by enumerating possible $i \in [n]$, the second inequality is by enumerating possible values of $T_i(t-1)$: $\{1, \dots, t-1\}$, the third inequality is by Chernoff-Hoeffding's inequality, and the last inequality is by $\sum_{t=1}^T \frac{1}{t^{\alpha-1}}  \leq \int_{1}^{+\infty} \frac{1}{t^{\alpha-1}} \leq \frac{1}{\alpha -2}$. Then by inequality \eqref{eq: D Rt(St)<= M} the proof is completed.
\end{proof}


Next, we show the regret of Part 3 is at most  $O(\log T)$.
\begin{lemma}\label{lem: regret4 bdd}
	For any $\epsilon_0>0$, the regret in Part 3 is bounded by
	$
	\E\left[ \sum_{t=1}^T  R_t(S_t)I_{\{ \bar E_t, B_t(\epsilon_0) \}}\right] \leq \frac{\alpha M n \log T}{2\epsilon_0^2}
	$
\end{lemma}
\begin{proof}
%	By Inequality \eqref{eq: D Rt(St)<= M} and the fact $I_{\{ \bar E_t, B_t(\epsilon_0) \}} \geq 0$, we have
%$
%	\E \sum_{t=1}^T  R_t(S_t)I_{\{ \bar E_t, B_t(\epsilon_0) \}} \leq M \E \sum_{t=1}^T  I_{\{  B_t(\epsilon_0) \}} 
%$.
	By the definition of $B_t(\epsilon_0)$ in \eqref{eq:Btepsilon}, whenever $B_t(\epsilon_0)$ happens, the algorithm  selects an arm $i$ that has not been selected for $\frac{\alpha \log T}{2\epsilon_0^2}$ times, increasing the selection time counter $T_i(t)$ by one. Hence, $ B_t(\epsilon_0) $ can happen for at most $\frac{\alpha n \log T}{2\epsilon_0^2}$ times. Then, by inequality \eqref{eq: D Rt(St)<= M}, the proof is completed.
\end{proof}

When $\bar E_t$ and $\bar B_t(\epsilon_0)$ happen (Part 4),  every selected arm is fully explored and every arm's sample average is within the confidence interval. As a result,  CUCB-Avg selects the right subset and hence contributes zero regret. This is formally stated in the following lemma. 


\begin{lemma}\label{lem: no regret bar E bar B}
	
	There exists $\epsilon_0>0$, such that for each $1\leq t\leq T$, if $\bar E_t$ and $\bar B_t(\epsilon_0)$ happen,  CUCB-Avg selects an optimal subset and $\E\!\left[ R_t(S_t)I_{\{ \bar E_t,\bar B_t(\epsilon_0) \}} \right]=0$. Consequently, the regret in Part 4 is 0.
\end{lemma}
\nit{Proof Sketch:} We defer the proof to Appendix \ref{aped: D no regret Ass} and \ref{aped: D no regret} and sketch the proof ideas here, which is based on two facts: \\
Fact 1: when $\bar E_t$ and $\bar B(\epsilon_0)$ happen, the upper confidence bounds can be bounded by
$ U_i(t)>p_i$ for all $i\in [n]$,
and the confidence bounds of the selected arm $j$ satisfy
$$ 
\left|\bar p_j(t-1) -p_j\right|<\epsilon_0, \ U_j(t)<p_j + 2\epsilon_0, \ \forall\, j \in S_t.$$
Fact 2: when $\epsilon_0$ is small enough, CUCB-Avg  selects an optimal subset.

To get the intuition for Fact 2, we consider the expression of $\epsilon_0$ in \eqref{equ: def epsilon} under Assumption (A1) (A2) in Proposition \ref{prop: A1A2 epsilon0}. Let  $\phi(p,D)=\{\sigma(1),\dots, \sigma(k)  \}$ denote the  optimal subset. In the following, we roughly explain why the selected subset $S_t$ is optimal given $\epsilon_0$ defined in \eqref{equ: def epsilon}:
%\begin{enumerate}
%	\item[i)]

	i) By $\epsilon_0 \leq \frac{\Delta_k}{2}$, we can show that the selected subset $S_t$ is either a superset or a subset of the optimal subset $\{\sigma(1),\dots, \sigma(k)  \}$.
	
	%\item[ii)]
	ii) By $\epsilon_0 \leq \delta_1/k$, we can show that we will not select more than $k$ arms, because, informally, even if  we underestimate $p_i$, the sum of arms in $\{\sigma(1),\dots, \sigma(k)  \}$ is still larger than $D-1/2$.
	
%	\item[iii)] 
iii) By  $\epsilon_0 \leq \delta_2/k$, we can show that we will not select less than $k$ arms, because, informally, even if  we overestimate $p_i$, the sum of  $k-1$ arms in $\{\sigma(1),\dots, \sigma(k)  \}$ is still smaller than $D-1/2$.
%\end{enumerate}
\qed

%Therefore, $S_t$ must be optimal. \qed%  $S_t=\{\sigma(1),\dots, \sigma(k)  \}$ by Line 7 of Algorithm \ref{alg: ucb_avg}.


The proof of Theorem \ref{thm: regret bdd D} is completed by summing up the regret bounds of Part 1-4.








==> arxiv submit/sec5_Dt.tex <==
\section{Time-varying target}\label{sec:time_varying}
In practice,  the load reduction target is usually time-varying. We will study the performance of CUCB-Avg in the time-varying case below. %Thus, it is worth studying the performance of CUCB-Avg given the time-varying target. 
%In the following, we will study the performance of CUCB-Avg in the time-varying case.

%Firstly, when the target $D_t$ changes with time, CUCB

%The adaptation of  Algorithm \ref{alg: ucb_avg} to the time-varying case is straightforward.
{\color{black}
Notice that CUCB-Avg can be directly applied to the time-varying case by using $D_t$ in Algorithm \ref{alg: ucb_avg} at each time step $t$. }%  At each time $t$, the decision maker uses the current target $D_t$ to run the algorithm  by letting $D=D_t$.  


Next, we  provide a regret bound for CUCB-Avg in the time-varying case. Notice that we impose no assumption on $D_t$ except that it is bounded, which is almost always the case in practice.
\begin{assumption}\label{ass: Dt bdd}
	There exists a finite $\bar{D}>0$ such that
	$0< D_t \leq \bar D, \ \forall \ 1\leq t\leq T$.
\end{assumption}

\begin{theorem}\label{thm: Dt regret bound}
	Suppose Assumption \ref{ass: Dt bdd} holds. When $T>2$, for  any $\alpha>2$, the regret of CUCB-Avg is  bounded by
	\begin{align*}
	\textup{Regret}(T)&\leq \bar M  n+ \frac{2\bar Mn}{\alpha -2} 
	+ \frac{\alpha \bar M n \log T}{2\epsilon_1^2}\\
	& + 2n^2 \sqrt{2\alpha \log T}\sqrt{T+ \frac{\alpha  \log T}{2\epsilon_1^2}},
	\end{align*}
	where  $\bar M = \max(\bar D^2, n^2)$, $\epsilon_1= \min( \frac{\Delta_{\text{min}}}{2}, \frac{\beta_{\text{min}}}{n})$, $\Delta_{\text{min}}= \min\{\Delta_i \mid 1\leq i \leq n-1, \Delta_i>0\}$ and $\beta_{\text{min}} = \min\{p_i \mid 1\leq i \leq n , p_i>0\}$.
\end{theorem}

%\textcolor{red}{How to show that my algorithm depends polynomially on $K$? By $\bar M=K_t^2$ I think}

Before the proof, we make a few comments below.



{\color{black}
\nbf{Dependence on $T$.} The bound is $O(\sqrt{T \log T})$, still sublinear in $T$, meaning that our algorithm learns the customers' response probabilities well enough to yield diminishing average regret in the time-varying case.

%The regret bound in Theorem \ref{thm: Dt regret bound} is $O(\sqrt{T \log T})$, which is worse than the $O(\log T)$ bound in the time-invariant case. We will provide intuitions behind this difference and the $O(\sqrt{T \log T}) $ bound. 

The  dependence on $T$ is worse than the static case which is $O(\log T)$. We briefly discuss the intuition behind this  difference.
In the proof of Theorem \ref{thm: regret bdd D}, we show that there exists a threshold $\epsilon_0$ depending on $D$ such that when the estimation errors of parameter $p_i$ for $i\in S_t$ are below $\epsilon_0$, our algorithm selects the optimal subset (Lemma \ref{lem: no regret bar E bar B}). Moreover, we also show that as $t$ increases, with high probability the estimation error will decrease and eventually our algorithm will find the optimal subset and generate no more regret. % such that our algorithm selects the optimal subset when the estimation error of the true parameter $p_i$ is smaller than $\epsilon_0$. SOur algorithm gradually decreases the estimation error to 0, so eventually the estimation error will go below $\epsilon_0$ with high probability. 
However, in the time-varying case the argument above no longer holds because the threshold $\epsilon_0$ will change with $D_t$, denoted as $\epsilon_0(D_t)$, and it is possible that the estimation error will always be larger than $\epsilon_0(D_t)$, as a result the algorithm may not find the optimal subset with high probability even when  $t$ is large. This roughly explains why the bound of the time-varying case  is worse than that of the static case. 

%denoted as $\epsilon_0(D_t)$ and , so in the worst case scenario, our algorithm may never provide estimation error below $\epsilon_0(D_t)$ if $\epsilon_0(D_t)$ decreases faster than the decay rate of the estimation error. This roughly explains why the time-varying case bound is worse than the static case. 

In addition, we provide some intuitive explanation for the scaling  $O(\sqrt{T \log T})$. It can be shown that  the regret at time $t$ is almost bounded by the estimation error at time $t$ under some conditions (Lemma \ref{lem: Sst under assumption Dt}). Since the estimation error is roughly captured by our confidence interval in \eqref{eq:Ui}, which  scales like $O(\sqrt{\log T/t})$,  the total regret scales like $ \sum_{t=1}^T O(\sqrt{\log T/t}) = O(\sqrt{T\log T})  $.



}
Finally, we note that the regret bound is for the worst-case scenario and  the  regret in practice may be smaller.


\nbf{Dependence on $n$.} The bound is polynomial on the number of arms $n$: $O(n^3)$ by $\bar M \sim O(n^2)$, demonstrating that our algorithm  can learn a large number of arms effectively in the time-varying case. Improving the cubic dependence on $n$ is left as future work.

\nbf{Role of $\epsilon_1$.} Notice that $\epsilon_1$ only depends on $p$ and does not depend on the target $D_t$. Roughly speaking, $\epsilon_1$ captures how difficult it is to rank the arms correctly by the value of $p_i$, in the sense that as long as the estimation error of each $p_i$ is smaller than $\epsilon_1$, the rank based on the estimation will be the correct rank based on the true parameter $p_i$. %Unlike $\epsilon_0$ in the static case, when the estimation error is smaller than $\epsilon_1$, the regret may still be positive, because even given the correct rank of the arms, the algorithm may still select a wrong number of arms.  

%$\epsilon_1$ is similar to $\epsilon_0$ in Theorem~\ref{thm: regret bdd D} for the static D case but has different properties. Notice that $\epsilon_1$ only depends on $p$ and does not depend on the target $D_t$. Roughly speaking, $\epsilon_1$ captures how difficult it is to rank the arms correctly by the value of $p_i$, in the sense that as long as the estimation error of each $p_i$ is smaller than $\epsilon_1$, the rank based on the estimation will be the correct rank based on the true parameter $p_i$. 
%Unlike $\epsilon_0$ in the static case, when the estimation error is smaller than $\epsilon_1$, the regret may still be positive, because even given the correct rank of the arms, the algorithm may still select a wrong number of arms. Nevertheless, the regret can be bounded  given a small estimation error (Lemma \ref{lem: Sst under assumption Dt}). This is the key property to establish the regret bound. 
%\textcolor{red}{Firstly, we note here that $\epsilon_1$ is a conservative measure in order to handle the time-varying $D_t$.} 

%\vspace{4pt}

%\nbf{Discussion of $\bar M$.}
%We note that $\bar M$ is the upper bound on the single-step regret $R_t(S_t)$ given any possible target $D_t$ and realization of $X_{t,i}$. Note that it is a conservative bound in order to handle the time-varying $D_t$.




\textcolor{black}{\subsection{Proof of Theorem \ref{thm: Dt regret bound}}}
Most parts of the proof is similar to the static case. We also consider $D_t\geq 1/2$ without loss of generality due to Corollary \ref{cor: D<1/2}. Besides, we also  divide the time steps into four parts and complete the proof by summing up the regret bound of each part. The first three parts can be bounded in  similar ways as the static case. The major difference comes from the Part 4.



(1) Initialization: the regret can be bounded by $\bar M n$ because the initialization at most lasts for $n$ time steps and $\bar M$ is an upper bound of the single-step regret.
% since D>0, it at least selects 1 arm in initialization.


(2) When $E_t$ happens: 
notice that Lemma \ref{lem: regret 1bdd} still holds in the time-varying case if we replace $M$ with $\bar M$, so the second part is bounded by
$
\E \sum_{t=1}^T I_{E_t} R_t(S_t)\leq \frac{2\bar Mn}{\alpha -2}
$.

(3) When $\bar E_t$ and $B_t(\epsilon_1)$ happen:
notice that Lemma \ref{lem: regret4 bdd} still holds so
$
\E \sum_{t=1}^T  R_t(S_t)I_{\{ \bar E_t, B_t(\epsilon_1) \}} \leq \frac{\alpha \bar M n \log T}{2\epsilon_1^2}
$.

(4) When $\bar E_t$ and $\bar B_t(\epsilon_1)$ happen, we can show that the regret is $O(\sqrt{T \log T})$ as stated in the lemma below.
\begin{lemma}\label{lem: regret4 Dt bound}
	The regret in Part (4) can be bounded by
$$	\E \sum_{t=1}^T  R_t(S_t)I_{\{ \bar E_t,\bar B_t(\epsilon_1) \}} \leq 2n^2\sqrt{\frac{\alpha \log T}{2}}  \sqrt{T+\frac{\alpha \log T}{2\epsilon_1^2}}. $$
\end{lemma}

\begin{proof}%Without loss of generality, we  consider $D_t\geq 1/2$ for all $t$, because if $D_t<1/2$ for some $t$, the algorithm will select the empty set and produce no regret at $t$.
	
	
%Below is the intuition behind the proof.

Our proof relies on the following lemma which shows that the regret at time $t$ can roughly be  bounded by the estimation error $\epsilon$ at $t$ when $\epsilon\leq \epsilon_1$.  %Then, we  show that the estimation error, roughly captured by $\sqrt{\log T/T_i(t-1)}$, almost decays  as  $O(\sqrt{\log T/t})$. Thus, the total regret is bounded by $\sum_t \sqrt{\log T/t}=\sqrt{T\log T}$.






%\nbf{Regret bound by the estimation error.}
%We show the regret bound when $ \bar E_t, \bar B_t(\epsilon)$ happens  is $O(\epsilon)$ for any $\epsilon\in (0,\epsilon_1]$. By definitions of $ \bar E_t, \bar B_t(\epsilon)$, this result means that the regret is at most $O(\epsilon)$ when the estimation error of the selected arms is at most $\epsilon$.
\begin{lemma}\label{lem: Sst under assumption Dt} 
	For any time step $t$,  consider any $D_t$ and any $0< \epsilon\leq \epsilon_1$ such that
	$\Pb(\bar E_t, \bar B_t(\epsilon))>0$.
	Let $\F_t$ denote the natural filtration up to time $t$. For any  $\F_{t-1}$ such that   $\bar E_t$ and $ \bar B_t(\epsilon)$ are true, 
 we have
$
	\E [R_t(S_t) \mid \F_{t-1}]\leq 2n \epsilon.%\label{equ: R(s)<2n xi}
$ %, where the expectation is  taken on the randomness only at stage $t$ since set $s$ is deterministic.
\end{lemma}
\nit{Proof sketch.}
Due to the space limit, we defer the proof to Appendix \ref{append: regret error if epsilon1>xi with assumption} and only sketch the proof here.  Firstly, we are able to show that under $\bar E_t$ and $\bar B_t(\epsilon)$, the selected subset differs from the optimal subset for at most one arm. This is mainly due to $\epsilon\leq \epsilon_1$. Secondly, we can bound the regret of the suboptimal selections by $O(\epsilon)$, which is mainly due to our quadratic loss function. \qed
%Due to space limit, we defer the proof to \citep{li2019CMAB} and only sketch the proof here. The proof relies on two facts. Firstly, we are able to show that under $\bar E_t, \bar B_t(\epsilon)$, the selected subset differs from the optimal subset for at most one arm. The intuition behind this is that in event $\bar E_t, \bar B_t(\epsilon)$, the estimation error is bounded by $\epsilon$. Since   $\epsilon\leq \epsilon_1\leq \Delta_{\text{min}}/2$ and  $\bar E_t, \bar B_t(\epsilon)$, the estimation error  $\epsilon$ is smaller than $\Delta_{\text{min}}$, then it can shown that the arms can be ranked correctly. In addition, by requiring $\epsilon\leq \epsilon_1\leq \beta_{\text{min}}/n$, it can be shown that our algorithm can at most select one more or one less arm under the correct order.


%Secondly, we are able to bound the regret of the suboptimal selections by $O(\epsilon)$. Intuition behind this bound is that our objective function is quadratic, and the regret of a near optimal subset can be approximated by, roughly speaking, the function value multiplied by the optimality gap generated by the near optimal subset. It can be shown that the function value can be bounded by $\epsilon$ and the optimality gap can be bounded by 1.



%\nbf{Finish the proof by bounding  the estimation errors.}
%When $D_t\leq 1/2$, the problem is trivial because the optimal selection is to select nobody. Therefore, we will 
Next, we will finish the proof by bounding the estimation errors. We introduce  event $H_t^q$ to represent that each selected arm $i$ at time $t$ has been selected for more than $
\frac{\alpha \log T}{2\epsilon_1^2}+q $ times for  $q=0, 1, 2, \dots$:
	$$H_t^q\coloneqq \left\{ \forall\, i\in S_t,  T_i(t-1) > \frac{\alpha \log T}{2\epsilon_1^2}+q \right\} \cap \bar E_t \cap \bar B_t(\epsilon_1).$$


%What's the intuition of the proof? Write the intuition (the story I told Lina.) Also, write the intuition for defining this new event. Make sure people can understand by reading the intuition, without digging into the math details.


In addition, we define the estimation error $\eta_q$ by the confidence interval radius when an arm has been explored for  $\frac{\alpha \log T}{2\epsilon_1^2}+q-1$ times:
$
\frac{\alpha \log T}{2\eta_q^2}=\frac{\alpha \log T}{2\epsilon_1^2}+q-1
$,
that is, 
$
\eta_q = \sqrt{ \frac{\frac{\alpha \log T}{2}}{q -1+ \frac{\alpha \log T}{2\epsilon_1^2}}}
$.
%It is easy to see that $\eta_q \leq \eta_1$ and $\eta_1= \epsilon_1$. 
The proof is completed by:
	\begin{align*}
&\E\!\left[ \sum_{t=1}^T  R_t(S_t)I_{\bar E_t\cap \bar B_t(\epsilon_1)} \right] %= \E \sum_{t=1}^T  R_t(S_t)I_{H_t^0} \\
 = \sum_{q=1}^T \sum_{t=1}^T  \E\!\left[ R_t(S_t)I_{(H_t^{q-1} -H_t^q)}\right] \\
& \leq  \sum_{q=1}^T\sum_{t=1}^T 2n \eta_{q} \Pb(H_t^{q-1}-H_t^q) \\
& \leq  \sum_{q=1}^T 2n^2 \eta_{q} =  2n^2\sum_{q=1}^T\sqrt{ \frac{\frac{\alpha \log T}{2}}{q-1 + \frac{\alpha \log T}{2\epsilon_1^2}}}\\
& \leq 2n^2\sqrt{\frac{\alpha \log T}{2} }\int_{0}^{T}\sqrt{ \frac{1}{q-1 + \frac{\alpha \log T}{2\epsilon_1^2}}}\ \mathrm{d}q\\
& \leq 4n^2\sqrt{\frac{\alpha \log T}{2}}  \sqrt{T+\frac{\alpha \log T}{2\epsilon_1^2}},
\end{align*}
where the first  equality is by $ \bar E_t \cap \bar B_t(\epsilon_1)=\cup_{q=1}^T (H_t^{q-1}-H_t^q)$;  the first inequality is by taking conditional expectation on $H_t^{q-1}-H_t^q$ and by  Lemma  \ref{lem: Sst under assumption Dt}, $(H_t^{q-1}-H_t^q) \subseteq \bar E_t \cap \bar B_t(\eta_q)$ and $\eta_q\leq \epsilon_1$; the second one is because
$H_t^{q-1}-H_t^q\subseteq\bigcup_{i=1}^n \{i \in S_t, \, T_i(t-1) = \frac{\alpha \log T}{2\epsilon_1^2}+q \}
$
and $\{i \in S_t, \, T_i(t-1) = \frac{\alpha \log T}{2\epsilon_1^2}+q \}$ occurs at most once; the third inequality uses the fact that $T>2$ and thus $ \frac{\alpha \log T}{2\epsilon_1^2}>1$.
\end{proof}

%\textcolor{red}{How to deal with $D_t<1/2$? Mention it somewhere!}




==> arxiv submit/sec6_simulation.tex <==




\begin{figure}
	\begin{subfigure}[b]{0.22\textwidth}
		\includegraphics[width=\textwidth]{regret_RI_10percent_avg.png}
		\caption{Average peak.}
		%	\label{fig:D}
	\end{subfigure} 
	\hfill
	\begin{subfigure}[b]{0.22\textwidth}
		\includegraphics[width=\textwidth]{regret_RI_10percent.png}
		\caption{Daily peak.}
		%\label{fig:Dt}
	\end{subfigure}
	\caption{The regret of CUCB, CUCB-Avg, and TS.}
	\label{fig: regret}
\end{figure}

\begin{figure}
	\begin{subfigure}[b]{0.22\textwidth}
		\includegraphics[width=\textwidth]{CI_RI_10percent_avg.png}
		\caption{Average peak.}
		%	\label{fig:D}
	\end{subfigure} 
	\hfill
	\begin{subfigure}[b]{0.22\textwidth}
		\includegraphics[width=\textwidth]{CI_RI_10percent.png}
		\caption{Daily peak.}
		%\label{fig:Dt}
	\end{subfigure}
	\caption{90\% confidence intervals of  load reduction's relative errors of CUCB-Avg (blue) and Thompson sampling (red).}
	\label{fig: conf interval}
\end{figure}
\begin{figure}
	\begin{subfigure}[b]{0.22\textwidth}
		\includegraphics[width=\textwidth]{D40_R20_T10e5_nto3500_2.jpg}
		\caption{When $T=10^5$}
		%	\label{fig:D}
	\end{subfigure} 
	\hfill
	\begin{subfigure}[b]{0.22\textwidth}
		\includegraphics[width=\textwidth]{D40T122R20nto3500.jpg}
		\caption{When $T=122$}
		%\label{fig:Dt}
	\end{subfigure}
	\caption{The regret of TS and CUCB-Avg for different $n$.}
	\label{fig: compare TS with diff. n}
\end{figure}


{\color{black}\section{Numerical Experiments}\label{sec: simulation}}
In this section, we conduct numerical experiments to complement the theoretical analysis above.% We compare the performance of our algorithm with CUCB and Thompson sampling (briefly introduced below) and discuss the effect of the tradeoff-parameter $\alpha$ and the number of customers.


%This section provides the results of numerical experiments to complement the analysis in the previous sections. First, we briefly introduce a classic algorithm in literature: Thompson sampling \citep{russo2017tutorial}. Then, we compare our CUCB-Avg  with  CUCB and Thompson sampling in two scenarios. In addition, we discuss the tradeoff between the exploration and exploitation and  the choice of algorithm parameter $\alpha$. Finally, we discuss the effect of the number of customers.



%In this section, we numerically study the performance of CUCB-Avg for residential DR, and compare it with classic bandit algorithms such as CUCB and Thompson sampling . We will show that CUCB-Avg performs much better than CUCB and similarly to Thompson sampling. 

%\subsection{A brief description of Thompson sampling}
%
%Thompson sampling  is a Bayesian algorithm that views the unknown probability vector $p$ as a random vector with a prior distribution, which is different from the algorithms in \ref{sec: online alg} which all view $p$ as an unknown but deterministic vector. Thompson sampling enjoys  good empirical performance in classical MAB problems \citep{chapelle2011empirical,agrawal2012analysis,gopalan2014thompson}, so it is worth comparing  our algorithm with Thompson sampling by simulation for our CMAB problem. The algorithm procedures are briefly summarized below. The algorithm first selects a subset $S_t = \phi(\hat p_t,D)$ based on a sample $\hat p_t$  from the prior distribution of $p$ at $t=1$ (or the posterior  distribution at $t\geq 2$ ), then updates the posterior distribution of $p$ by observations $\{X_{t,i} \}_{i\in S_t}$. For more details, we refer the reader to \citep{russo2017tutorial}.



\subsection{Algorithms comparison}\label{subsec: numerical Dt}
We will compare our algorithm with CUCB  \citep{chen2016combinatorial}, which is briefly explained in Section \ref{subsec: CUCB}, and Thompson sampling (TS), an algorithm with good empirical performance in classic MAB problems. In TS, the unknown parameter $p$ is viewed as a random vector with a prior distribution. The algorithm selects a subset $S_t = \phi(\hat p_t,D)$ based on a sample $\hat p_t$  from the prior distribution of $p$ at $t=1$ (or the posterior  distribution at $t\geq 2$), then updates the posterior distribution of $p$ by observations $\{X_{t,i} \}_{i\in S_t}$. For more details, we refer the reader to \citep{russo2017tutorial}. 


In our experiment, we consider a residential demand response program with 3000 customers. Each customer can either participate in the DR event by reducing 1kW  or not.  The probabilities of participation are i.i.d. $\text{Unif}[0,1]$. \textcolor{black}{The demand response events last for one hour on each day from June to September in 2018,} with a goal of shaving the 
 peak loads in Rhode Island. The \textit{hourly} demand profile is from New England ISO.\footnote{\url{https://www.iso-ne.com/isoexpress/web/reports/load-and-demand/-/tree/demand-by-zone}} We consider two schemes to determine the peak-load-shaving target $D_t$:
\begin{enumerate}
	\item[i)] Average peak: Compute the averaged  load profile in a day by averaging the  daily load profiles in the four months. The constant target $D$ is the 5\% of the difference between the peak load and the  load at one hour before the peak hour of the averaged load profile. %\textcolor{red}{this sentence is confusing and I don't understand. Can you explain it?}
	\item[ii)] Daily peak: On each day $t$, the target $D_t$ is 5\% of the difference between the peak load and the load at one hour before the peak hour of the daily demand.
\end{enumerate}



 In our algorithms, we set $\alpha=2.5$. In Thompson sampling, $p$'s prior distribution  is   $\text{Unif}[0,1]^n$. We consider one DR event per day and plot the daily performance. %The plots  are based on  100 simulations \textcolor{red}{(my current plot is only based on 5 iterationss)}. 


Figure \ref{fig: regret} plots the regret of CUCB, CUCB-Avg and TS under the two schemes of peak shaving. The x-axis is in log scale and the resolution is by day. Both figures show that CUCB-Avg  performs  better than  CUCB and  TS. In addition, the regret of CUCB-Avg in Figure \ref{fig: regret}(a) is linear with respect to $\log(T)$,  consistent with our theoretical result in Theorem \ref{thm: regret bdd D}. Moreover, the regret of CUCB-Avg in Figure \ref{fig: regret}(b) is almost linear with $\log(T)$, demonstrating that in practice the regret can be much better than our worst case regret bound in Theorem \ref{thm: Dt regret bound}. %which considers adversarially generated targets.


Figure \ref{fig: conf interval} plots the 90\% confidence interval of the relative  reduction error, $\frac{\sum_{i\in S_t}X_{t,i}-D_t}{D_t}$, of CUCB-Avg and TS by 1000 simulations. It is observed that the relative error of CUCB-Avg roughly stays within $\pm 5\%$,  much better than Thompson sampling. This again demonstrates the reliability of CUCB-Avg. Interestingly, the figure shows that TS tends to reduce less load than the target, which is possibly because TS overestimates the customers' load reduction when selecting customers.  \red{Finally, on August 18th both algorithms cannot fulfill the daily peak target because  it is very hot and the target is too high to reach even after selecting all the users. }


Finally, we compare TS and CUCB-Avg for different $n$ by considering the scheme (i). We consider two cases: 1) when $T$ is very large so the  regret is dominated by the $\log(T)$ term, 2) when $T$ is a reasonable number in practice. We let $T=10^5$ for case 1 and $T=122$ (the total number of days from June to September) for case 2. We consider a smaller target $D=40$ for illustration and consider $n=500:500:3500$. Figure \ref{fig: compare TS with diff. n}(a) shows that the dependence on $n$ of CUCB-Avg's regret is similar to  that of TS when $T$ is large, and the dependence is not cubic,  the theoretical explanation of which is left for future work. Moreover, Figure \ref{fig: compare TS with diff. n}(a) shows that CUCB-Avg can achieve better regrets than TS under a properly chosen small $\alpha$. Though not explained by theory yet,  the phenomenon that a small $\alpha$ yields good performance has been observed in literature \citep{wang2018thompson}. Further, Figure \ref{fig: compare TS with diff. n}(b) shows that CUCB-Avg achieves significantly smaller regrets than TS for a practical $T$, indicating the  effectiveness of our algorithm in reality. 



% large  that both algorithms cannot fulfill the reduction target. %both algorithms reduces much less demand than the target in Figure \ref{fig: conf interval}(b), which is because the target on this day is too high to be reached by selecting all customers. 
% To see this, consider same by determining the number of selected customers $k_t$ based on  with higher realization
%Figure \ref{fig:constant D}(b) and Figure \ref{fig:random walk}(b) plot the 90\% confidence interval of the relative load reduction error with respect to the target of CUCB-Avg and Thompson sampling by 1000 simulations of Scenario 3. Firstly, both figures show that the load reduction error of CUCB-Avg roughly stays within the 5\% error region of the   reduction target with a high probability after a few days; while the load reduction error by Thompson sampling is likely to stay outside the 5\% error region. This again demonstrates the reliability of CUCB-Avg. Secondly,  in Figure \ref{fig:random walk}(b), on August 18th both CUCB-Avg and Thompson sampling produces a much smaller load reduction than the target. This is because the peak load on August 18th is so high that even selecting all customers is not able fulfill the load reduction target. Finally, an interesting phenomenon is that Thompson sampling tends to reduce less load than required. One possible explanation is that Thompson sampling overestimates the true parameters when selecting customers due to the properties of order statistics. We provide intuitions behind this explanation by considering the simplest setting when all customers share the same true parameter $p_i$ and the same posterior distribution whose mean is the true parameter.  When we randomly generate $\hat p_i$ from the posterior distribution and select $k$ customers, on average the sum of $\hat p_i$ is $p_i k$. However, when applying Thompson sampling to our problem, the algorithm  selects top customers, and the top $k$ customers' sum of  is higher than $p_i k$ by applying the order statistics results.

%\footnote{Consider a simple setting where all customers have the same parameter $p_1$ and the same posterior distribution $\mathcal P$ with mean $p_1$.  Let $\hat p_i$ be randomly sampled from $\mathcal P$. Thompson sampling  selects the top  customers with highest $\hat p_i$. By the property of the order statistics, the $p_1 k$.} 

\subsection{More discussion on the effect of $\alpha$ and $n$}
{Figure \ref{fig: compare TS with diff. n} has  shown that the choice of $\alpha$ and $n$ affects the algorithm performance. In this subsection, we will discuss  the effect of $\alpha$ and $n$ in greater details. In particular, we will study the DR performance by the relative deviation of the load reduction, which is defined as $\sqrt{\E L(S_t)}/D_t$, for each day during the four months.  }

Figure \ref{fig:alpha} shows the relative deviation of CUCB-Avg for different $\alpha$ when $n=3000$ and when the target is determined by scheme (i) in Section \ref{subsec: numerical Dt}. It is observed that when $T$ is small, a large $\alpha$ provides smaller relative deviation, thus better performance. This is because   the information of customers is limited when $T$ is small, and larger $\alpha$ encourages exploration of the information, thus yielding better performance. When $T$ is large, a smaller $\alpha$ leads to a better performance. This is because when $T$ is large, the information of customers is sufficient, and a small $\alpha$ encourages the exploitation of the current information, thus generating better decisions. {The observations above are  also consistent with Figure \ref{fig: compare TS with diff. n}}. Further, Figure \ref{fig:alpha} shows that for a wide range of $\alpha$'s values, CUCB-Avg  reduces the deviation to below 5\% after a few days, indicating that CUCB-Avg is reasonably robust to the choice of $\alpha$. 

Figure \ref{fig: n} shows the relative deviation of CUCB-Avg for different $n$ when $\alpha=2.5$ and when the target is determined by scheme (i) in Section \ref{subsec: numerical Dt}. It is observed that even with a large number of customers, CUCB-Avg reduces the relative deviation to below 5\% very quickly, demonstrating that our algorithm can handle large $n$ effectively. In addition, when $T$ is small, a small $n$ provides smaller relative deviation, because a small number of customers is easier to learn in a short time period. When $T$ is large, a large $n$ provides better performance, because there are more reliable  customers to choose from a larger customer pool. {It is worth mentioning that though Figure \ref{fig: compare TS with diff. n}(a) shows that the regret increases with  $n$ when $T$ is large, there is no conflict because the regret captures the gap between the  deviation generated by the algorithm and  the optimal one, which may increase even when the algorithm generates less deviation since the optimal deviation also decreases. }% and even the value of deviation decreases, the gap between the deviation and the optimal one may still increase.


\begin{figure}
	\centering
		\includegraphics[width=0.3\textwidth]{different_alpha.png}
	\caption{Effect of $\alpha$}
		\label{fig:alpha}
\end{figure}

\begin{figure}
	\centering
	\includegraphics[width=0.3\textwidth]{different_n_avg.png}
		\caption{Effect of $n$}
	\label{fig: n}
\end{figure}


\subsection{On the user fatigue effect}

It is widely observed that customers tend to be less responsive to demand response signals after participating in DR events consecutively. This effect is usually called \textit{user fatigue}. Though our algorithm and theoretical analysis do not consider this effect for simplicity, our CUCB-Avg can handle the fatigue effect after small modifications, which is briefly discussed below.% To show how to do it, we provide some details below. 
%And in numerical experiments, our CUCB-Avg can work reasonably well after small simple and direct modifications  when the user fatigue effect is considered. The numerical experiments and results are provided below. Theoretical analysis is left for future work.


For illustration purpose, we consider a simple model of user fatigue effect.  Each customer $i$ is associated with an original response probability $p_i$. The response probability at stage $t$, denoted as $p_i(t)$, decays exponentially with a fatigue ratio $f_i$ if customer $i$ has been selected consecutively, that is,  $p_i(t)=(f_i)^{\chi_i(t)} p_i$ if customer $i$ has been selected from day $t-\chi_i(t)$ to day $t-1$. If the customer is not selected , we consider that the customer takes a rest at this stage and will respond to the next DR event with the original probability. Though the fatigue model may be too pessimistic about the effects of the consecutive selections by considering exponential decaying fatigue factors,  and too optimistic about the relaxation effect by assuming full recovery after one day rest, this model captures the commonly observed phenomena that the consecutive selection is  a key reason for user fatigue and customers can recover from fatigue if not selected for some time \citep{hopkins2017best}. The model can be revised to be more complicated and realistic, which is left as future work. 


Next, we explain how to modify CUCB-Avg to address the user fatigue effects. We consider that the aggregator has some initial estimation of the fatigue ratio of customer $i$, denoted as $\tilde f_i$, and will use the estimated fatigue ratios to rescale the upper confidence bounds and sample averages in Algorithm 2 to account for the fatigue effect. In particular, the rescaled upper confidence bound is $(\tilde f_i)^{\chi_i(t)}U_i(t)$, and the rescaled history sample average is $\bar p_i(t)= \frac{1}{T_i(t)}\sum_{\tau \in I_i(t)} \frac{X_{\tau, i}}{(\tilde f_i)^{\chi_i(t)}}$, where $\chi_i(t)$ denotes the number of consecutive days up until $t-1$ when customer $i$ is selected.


In our numerical experiments, different users may have different user fatigue ratios, which  are generated i.i.d. from $\text{Unif}[0.75, 0.95]$. % the parameters are chosen based on the pilot studies by ThinkEco ( \blue{Q: what's the ppt numbers? I didn't findi it?} \blue{Q: how to cite private data? I think Adam has a paper on it}). 
Other parameters are  the same as  in Section 6.1. Figure \ref{fig: consumer fatigue} plots the relative deviation of our modified CUCB-Avg in two scenarios: i) the aggregator  has access to the accurate fatigue ratio, i.e. $\tilde f_i=f_i$; ii) the aggregator only has a rough estimation for the entire population: $\tilde f_i =0.85$ for all $i$. It can be observed that our algorithm is able to reduce the relative deviation to below 5\% after a few days even when the fatigue ratios are inaccurate. This demonstrates that our algorithm, with some simple modifications, can work reasonably well even when considering customer fatigue effects. %We leave more discussion and theoretical analysis and better algorithm design as future work.




\begin{figure}[htp!]
	\centering
	\includegraphics[width=0.3\textwidth]{consumer_fatigue.jpg}
	\caption{The performance of our CUCB-Avg (after simple modifications) when considering user fatigue.}
	\label{fig: consumer fatigue}
\end{figure}




==> arxiv submit/sec7_conclusion.tex <==
\section{Conclusion}
This paper studies  a CMAB problem  motivated by residential demand response with the goal of minimizing the difference between the total load adjustment and the target value. 
 We propose  CUCB-Avg and show that CUCB-Avg achieves sublinear regrets in both static and   time-varying cases. 
 There are several interesting directions to explore in the future. First, it is  interesting to improve the dependence on $n$. Second, it is worth  studying the regret lower bounds.   Besides, it is worth considering more realistic behavior models which may include e.g. the effects of temperatures and humidities, the user fatigue, correlation among users,  time-varying response patterns, general load reduction distributions, dynamic population, etc. % is also worth studying. 
 
 
 
 %other load reduction distributions such as continuous distributions and even Markov processes. It is also worth studying  the lower bound
%Future work includes  considering  dynamic population, more realistic customer behavior models that involve the effect of temperature and humidity, user fatigue, correlation among users, time-varying response probabilities, other load reduction distributions such as continuous distributions and even Markov processes. It is also worth studying  the lower bound

 %general customer behavior models, e.g.  continuous distributions, Markov processes, etc., time-varying response probabilities, 


